History Encoding Representation Design for Human Intention Inference

In this extended abstract, we investigate the design of learning representation for human intention inference. In our designed human intention prediction task, we propose a history encoding representation that is both interpretable and effective for prediction. Through extensive experiments, we show our prediction framework with a history encoding representation design is successful on the human intention prediction problem.

==> part1_inside_policy/mbrl/sections/1Introduction.tex <==
\section{Representation Reasoning in RL based Autonomous Driving}

Autonomous driving in urban scenario is a complicated challenge that requires extensive surrounding environment recognition and decision making. The traditional rule-based methods often fail to accomplish satisfactory driving performance in highly complicated traffic scenarios due to the biased human-designed heuristics. On the other hand, massive data and computation power have advanced the performance of the learning methods in various fields of computer vision, data science, robotics and autonomous driving. In the field of autonomous diving, the most popular and studied learning based methods are imitation learning (IL) based, which essentially use neural network to do behavior cloning of the input-output combinations of the human expert drivers. One of the earliest attempts are the ALVINN \cite{pomerleau1989alvinn} and \cite{muller2006off}, and more recent works include \cite{nvidia2016end}, \cite{xu2016end}. Waymo has also applied IL to learn a urban driving policy from huge human driving data \cite{bansal2018chauffeurnet}. The progress over the years is mainly on using larger dataset and more sophisticated neural network structures. However, since the policies are still trained in a supervised manner, they are inevitably limited by the dataset. Chen et al sought to obtain a more stable policy by first learning a future trajectory and then have a low level controller to track the trajectory \cite{chen2019deep}.

However, the IL based methods are usually limited to the expert demonstration data and lack of generality capability. To summarize, the IL methods suffer from the following shortcomings:
\begin{enumerate}
    \item It requires collecting a large amount of driving data, which is costly and time consuming.
    \item The training dataset is biased compared to real world driving, since the expert drivers generally do not provide data for dangerous situations.
    \item IL essentially clones the human driver behavior, and cannot exceed the human performance.
\end{enumerate}

Compared with the rule-based and the IL methods, RL methods are more suitable for training autonomous driving policies because it can have the agent to explore and interact with the traffic environment without human guidance. Therefore, the policies trained can not only learn cases that are not in the IL training set, but also potentially exceed performance of the human drivers. Within the class of RL methods, there are two major categories:

\begin{enumerate}
\item Model-free RL, in which the reconstruction of a system dynamics model is not required. Model-free RL has been demonstrated capable of solving many challenging tasks such as continuous control based on state space \cite{lillicrap2015continuous,mnih2016asynchronous}, driving game with low-dimensional feature vector or image pixels as inputs \cite{sallab2016end}. For the application for driving,\cite{wolf2017learning}, learns the steer command in a simulator with discrete action space. Wayve's researchers use more sophisticated network and representation learning to use RL to drive an autonomous vehicle in urban scenarios \cite{kendall2019learning}. Chen et al work on model-free RL provided a benchmark comparison of different model free RL algorithms in the Carla simulator \cite{chen2019model}.

\item Model-based RL methods, in which optimal control is applied based on the inference of an approximation of the system dynamics function. Model-based RL lies in the intersection of model based planning, control and RL, which iteratively learns the model of the complex environment, and optimizes the control policy base on the understanding of the environment dynamics. The model-based RL have been proved capable of solving a number of complicated manipulation tasks \cite{levine2016end} and aerial vehicle \cite{zhang2016learning} in both simulator and real world.
\end{enumerate}

In general, model-free RL methods suffer from low sample efficiency and lack of interpretability. This is because the RL policy is trained in an end-to-end manner, and the structural information of the complicated driving scenarios cannot be modeled in a compact and representative way. On the other hand, in model-based RL an accurate approximation of the complicated system dynamics is required for accurate planning and control. The complication nature of the autonomous driving makes it challenging to model using a data-driven method. Therefore, selecting a suitable representation and adopting a suitable representation learning strategy inside the policy network (or inside the dynamics model) is of significance for the success of the policy learning using model-free RL (or model-based RL).

In the first half of this chapter (from Section \ref{sec:start} to Section \ref{sec:end}), we investigate the representation selection and representation learning strategies for solving an autonomous driving task based on model-based and model-free RL. For model-based RL, we propose to adopt a Gaussian mixture model to serve as a general global model, and adapt to a local linear Gaussian model to precisely capture the complicated autonomous driving system dynamics. For model-free RL, we design the graph neural network representation encoding so as to better extract the multi-entity relationship in urban autonomous driving.

==> part1_inside_policy/mbrl/sections/2Related_work.tex <==
\section{Autonomous Driving Problem Setup}
We model the autonomous driving task using a Markov Decision Process (MDP), whose state is defined using $s_t$, the agent interacts with the environment by taking actions $a_t$, derived using its control policy $\pi_\theta (a_t | s_t)$, and the control policy is parameterized by $\theta$. In autonomous driving, the MDP state can include the lane tracking status, speed of the autonomous vehicle, and the obstacle vehicles. The MDP action is the control command for the autonomous vehicle, corresponding to throttle, brake, and steering angle. Accepting the action of the agent, the environment would evolve in time according to the system dynamics $p(s_{t+1} | s_t, a_t)$. The system dynamics can be very complicated in general for the urban driving tasks given the dense traffic interaction. Furthermore, the obstacles movements are usually not controllable by the control commands of the autonomous vehicle.

With the system governed by the dynamics function and the control policy, the trajectory distribution can be described as a distribution of 

\begin{align}
\pi_\theta(\tau) = p(x_0) \prod_{t=0}^{T-1} \pi_\theta(a_t|s_t) p(s_{t+1}|s_t, a_t)
\end{align}

where $\tau=\{s_0, a_0, s_1, a_1, ..., s_T, a_T\}$. The goal of the autonomous driving task is described by a cost function, $l(s_t, a_t)$, which can be penalties for the lateral and reference speed deviation of the autonomous vehicle, or for the collisions with the obstacle. The overall objective would then be to minimize the expectation $E_{\pi_\theta(\tau)}[\Sigma l(s_t, a_t)]$, which we will abbreviate as $E_{\pi_\theta} [l(\tau))]$. It is noted that the problem formulation for RL is the same as that of the optimal control, only the system dynamics $p(s_{t+1}|s_t, a_t)$ is not known, and often very complex, such that one can not precisely model using mathematical equations, but can only use parametrized models to approximate it. This brings challenges to the learning of a driving policy, but also the setting can enable the RL policy to control the vehicle under complicated vehicle dynamics, and dense traffic that is hard to model.

\subsection{Carla Driving Simulation Settings}
\label{carla_setup}

We conduct our experimental validation using the Carla urban driving simulator \cite{dosovitskiy2017carla}, which is a high-fidelity open-source simulator by Intel.

\paragraph{For the model-based RL experiments}, due to the limitation of the policy optimization operation, we conduct experiments under three different scenarios, straight lane, $90\degree$ turning, and circular roundabout. And for each scenario, we investigate the performance of the proposed method and a series of baseline algorithms with and without obstacle vehicles. The Carla simulator and the simulated scenarios are shown in Fig. \ref{fig:carla}. In order to test the performance of the RL methods serving as motion planner, we directly extracted the vehicles and map states from the Carla simulator, which is input to the model-based RL policy. Because the RL policy take in fixed dimensional states, we designed two kinds of states for the scenarios with and without obstacles. For the tasks without obstacles, the state input include the lateral deviation and yaw error of the autonomous vehicle with respect to the road block, and the velocity of the autonomous vehicle. For the cases with obstacles, in order to maintain fixed state dimension, we investigate only the influence of the front vehicle, and augment the state of the relative position and velocity between the autonomous vehicle and the front vehicle to the previously defined state, to obtain the state for these cases. 

\begin{figure}[t]
\centering
\includegraphics[width=0.7\linewidth]{part1_inside_policy/mbrl/figures/carla.png}
\caption{The Carla urban driving simulator. Upper Left: the ego view of the autonomous vehicle; Upper Right: the roundabout experiment setting; Lower Left: the 90$\degree$ turning experiment setting; Lower Right: the straight driving experiment setting.}
\label{fig:carla}
\end{figure}

\paragraph{For the model-free RL experiments}, since the policy is learned in an end-to-end manner, we are able to learn a more general policy that drives the ego vehicle around within the simulated town. There are 100 surrounding vehicles that are controlled using the intelligent driver models (IDM) randomly generated inside the simulator, and the ego vehicle could encounter some of them during its navigation. We can extract various kinds of state observations from the simulator, such as the front view camera image, the simulated lidar observation and the state vectors for the surrounding vehicles. We can also design and render a block representation of the local traffic environment for better visualization. Fig. \ref{fig:carla_obs} shows the block representation and the simulated sensor observations of the driving setting.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{part1_inside_policy/mbrl/figures/carla_obs.png}
\caption{Block representation and the simulated sensor observations of the Carla driving setting. Left: the block representation showing the ego vehicle (red), surrounding vehicles (green) and the road map; Middle: the simulated lidar observation; Right: the front view camera image.}
\label{fig:carla_obs}
\end{figure}

We also designed concise and effective cost functions to model the objective of the driving tasks. For the road block tracking without considering the obstacle, we define the tracking cost to be

\begin{align}
c_t(s_t, a_t) = \alpha_l \Delta y^2 + \alpha_y \Delta \phi^2 + \alpha_v (v-v_{ref})^2 + \alpha_a a^2 + \alpha_\sigma \sigma^2
\end{align}

where $\Delta y$ is the lateral deviation, $\Delta \phi$ is the yaw angle error, $v$ is the velocity of the autonomous vehicle, $v_{ref}$ is the reference speed for the tracking, $a$ is the acceleration action, and $\sigma$ is the steering action.

When considering the obstacle, we designed a nonlinear cost function that only takes effect when the autonomous vehicle is within the same lane of the obstacle vehicle, and the distance $s$ is smaller than 20m, where we add the additional term of

\begin{align}
c_{aug}(s_t, a_t) = \beta_s (20-s) + \beta_v v_{approach}
\end{align}

where $v_{approach}$ is the approaching speed of the ego and obstacle vehicle. If there is a collision of between the ego vehicle and an obstacle vehicle, a large penalty is given and the episode is terminated. The reward function for the MDP and for RL is the negative of the cost function.


%Most literature on using deep learning to solve autonomous driving problems is based on IL, which essentially use neural network to do behavior cloning of the input-output combinations of the human expert drivers. One of the earliest attempts are the ALVINN \cite{pomerleau1989alvinn} and \cite{muller2006off}, and more recent works include \cite{nvidia2016end}, \cite{xu2016end}. Waymo has also applied IL to learn a urban driving policy from huge human driving data \cite{bansal2018chauffeurnet}. The progress over the years is mainly on using larger dataset and more sophisticated neural network structures. However, since the policies are still trained in a supervised manner, they are inevitably limited by the dataset. Our previous work sought to obtain a more stable policy by first learning a future trajectory and then have a low level controller to track the trajectory \cite{chen2019deep}.

%Model based RL has been demonstrated to be capable of solving many challenging tasks including in control \cite{lillicrap2015continuous,mnih2016asynchronous}. Various deep RL methods including deep Q-learning and actor-critic algorithms have been applied to train lane keeping policies with low-dimensional feature vector or image pixels as inputs \cite{sallab2016end}. Another deep Q learning application is \cite{wolf2017learning}, which learns the steer command of an autonomous vehicle in simulation with discrete action space. Wayve's researchers used more sophisticated network and representation learning to use RL to drive an autonomous vehicle in urban scenarios \cite{kendall2019learning}. Our previous work on model free RL provided a benchmark comparison of different model free RL algorithms in the Carla simulator \cite{chen2019model}.

%However, as is pointed out, the model free reinforcement learning suffers from great sample inefficiency\cite{xu2017cascade, xu2019toward}. Also, since the neural network policies are trained in an end to end manner, it lacks of interpretability and can be very hard to transfer the real world vehicles \cite{xu2018zero, tang2019disturbance}. The model based or policy search based RL are more sample efficient and have been proved capable of solving a number of complicated manipulation tasks \cite{levine2016end} and aerial vehicle \cite{zhang2016learning} in both simulator and real world. In addition to the guided policy search method \cite{levine2013guided}, we also test and compare it to one of the most popular policy search method of cross entropy method \cite{de2005tutorial} to validate the effectiveness of the proposed method in urban autonomous driving.

==> part1_inside_policy/mbrl/sections/3Methodology.tex <==
\section{Model-based RL: Dynamics Representation and Policy Optimization}

The model-based RL method we adopt is a RL method that combines the strengths of both RL and optimal control. The algorithm follows the formulation is as shown in Fig. \ref{fig:gps_structure}. The model-based RL algorithm iteratively updates the belief of the system dynamics model and to optimize the control policy under the current dynamics approximation function. The two steps are called the system dynamics learning step and the policy optimization step. Our algorithm shares a similar framework of the guided policy search (GPS) \cite{levine2013guided}, but we don't learn an imitation neural network of the optimization based policy, although we still refer to our algorithm as a variant of GPS. For the system dynamics learning step, the agent first explores the environment and collects trajectory samples of $\tau=\{s_0, a_0, s_1, a_1, ..., s_T, a_T\}$. The collected data tuples $(s_t, a_t, s_{t+1})$ are then used to learn the system dynamics function $p(s_{t+1}|s_t, a_t)$. This is a supervised learning process, optimizing the objective of:

\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{part1_inside_policy/mbrl/figures/gps.png}
\caption{The framework of our proposed model-based RL method. For each iteration, we first collect trajectories in the simulator using the current policy, then the trajectory samples are used to update the system dynamics approximator, which is further used as the model within the model-based policy optimization.}
\label{fig:gps_structure}
\end{figure}

\begin{align}
\max_{p(s_{t+1}|s_t, a_t)} p(\tau)
\end{align}

The policy optimization step learns the optimal policy $\pi_\theta(a_t|s_t)$ based on the learned dynamics $p(s_{t+1}|s_t, a_t)$, in order to obtain an optimal return $E_{\pi_\theta} [l(\tau))]$. There is a large amount of freedom in the representation formulation and the representation learning strategy selections. In our autonomous driving application, we select the system dynamics representation to be a Gaussian mixture models adopt the idea of local models in order to get high sample efficiency. Concretely, a time-varying linear-Gaussian model is applied to approximate the local behavior of the system dynamics. Therefore, the learned system dynamics model shall follow the following formulation:

\begin{align}
p(s_{t+1}|s_t, a_t) = \mathcal{N} (A_t s_t+B_t a_t +f_t, F_t)
\end{align}

Similarly, the policy model is also represented using a linear Gaussian model, denoted as:

\begin{align}
\pi_\theta(a_t|s_t) =  \mathcal{N} (K_t s_t+k_t, C_t)
\end{align}

The local linear models can be learned very efficiently with a small number of samples, but they can only describe the local properties of the nonlinear functions. Therefore, in the following the policy optimization step, the new trajectory produced by the new policy, denoted $\tau$, shall not be too far in distribution to the old trajectory samples we used to learn dynamics $p(s_{t+1}|s_t, a_t)$, so as to guarantee the modeling representation accuracy of the local linear model. We denote the old trajectories using $\hat{\tau}$. We adopt the KL-divergence to describe the change of the trajectory distributions, then the policy optimization process can be modeled using the optimization problem below.

\begin{align}
\min_\theta E_{\pi_\theta} [l(\tau))]
\end{align}
\begin{align}
\text{s.t. } D_{KL} (p(\tau)\|p(\hat{\tau}))<\epsilon
\end{align}

In the two following subsections, we elaborate the details of the representation selection and usage in the system dynamics learning step and the policy optimization step.

\subsection{System Dynamics Learning}
The goal of the system dynamics learning is not only to learn a precise local linear function, but also to learn it highly sample efficiently. Therefore, we adopt a global model as the prior, which evolves throughout the whole model-based RL lifetime, and fit the local linear dynamics to it at each iteration. The global prior itself does not need to be a good approximation, it only needs to capture the major property of the system dynamics, such as to increase the regression sample efficiency. This approach shares a similar idea with model agnostic meta learning (MAML) \cite{finn2017model}, where the prior model is not an accurate approximation of the dynamics, but after a fast adaptation process the updated model could capture more precise dynamics properties.

In the case of autonomous driving, there are naturally a series of different driving patterns. Within each driving pattern, the dynamics models follow a similar property. Therefore, we adopt the Gaussian mixture model (GMM) to serve as the nonlinear prior model, with each mixture element serving as prior for one driving pattern. Under this setting, each tuple sample $(s_t, a_t, s_{t+1})$ is first assigned to a pattern, and then used to update the mixture element. This process is a typical Expectation Maximization (EM) process used to train a GMM. Finally, at each iteration, we fit the current episode of data tuples $\{(s_t, a_t, s_{t+1})\}$ to the GMM, incorporating a normal-inverse-Wishart prior. The local linear dynamics $p(s_{t+1}|s_t, a_t)$ is derived by conditioning the Gaussian on $(s_t, a_t)$.

\subsection{Policy Optimization}

In order to solve for the policy optimization, we incorporate a popular gradient based method for constrained optimization, the dual gradient descent (DGD), which is summarized in algorithms \ref{algo:gps}. The main idea of the DGD is as follows. We first write out the Lagrangian:

\begin{align}
L(\theta, \lambda) = \sum_{t=0}^{T-1} E_{\pi_\theta} [l(s_t, a_t) + \lambda (D_{KL}(p(\tau)\|p(\hat{\tau}))-\epsilon)]
\end{align}

,where
\begin{align}
D_{KL}(p(\tau)\|p(\hat{\tau})) = E_{\pi_\theta} [log(p(\tau))-log(p(\hat{\tau}))]
\end{align}

The DGD trick is to first minimize the Lagrangian function under fixed Lagrangian multiplier $\lambda$, and then increase the $\lambda$ penalty if the constrained is violated, so that more emphasis is placed on the constraint term in the Lagrangian function in the next iteration. We can reformulate the minimization of the Lagrangian function to be some trajectory optimization problem with regard to some augmented cost function $c(s_t, a_t) = l(s_t, a_t)/\lambda - log(p_{\hat{\tau}}(a_t, s_t))$, where $l(s_t, a_t)$ is the original MDP step cost. The optimization is therefore updated to:

\begin{align}
\min_{\pi_\theta} \sum_{t=0}^{T-1} c(s_t, a_t)
\end{align}

Since we can directly compute the cost function $c(s_t, a_t)$ and its derivatives, we can then solve the trajectory optimization problem using linear quadratic Gaussian (LQG) \cite{aastrom2012introduction}. After the Lagrangian is optimized under a fixed $\lambda$, in the second step of DGD, $\lambda$ is updated using the function below with step size $\alpha$:

\begin{align}
\lambda \leftarrow \lambda+\alpha(D_{KL}(p(\tau)\|p(\hat{\tau}))-\epsilon))
\end{align}

, and the DGD loop is closed.

\begin{algorithm}[H]
\SetAlgoLined
Constrained optimization problem defined by (5-6)\\
Initialize $\lambda=\lambda_{0}$, $itr=0$\\
\While{$itr < maxIteration$}{
  Rewrite $L(\theta, \lambda)$ to $\sum_{t=0}^{T-1} c(s_t, a_t)$\\
  Solve for optimal $\pi_\theta$ using LQR\\
  Evaluate constraint violation $\Delta = D_{KL}(p(\tau)\|p(\hat{\tau}))-\epsilon)$\\
  Update $\lambda \leftarrow \lambda+\alpha\Delta$
}
\caption{Dual Gradient Descent for Policy Optimization}
\label{algo:gps}
\end{algorithm}

==> part1_inside_policy/mbrl/sections/4Experiment_Setup.tex <==
\subsection{Compared Methods}

We refer to our method as GPS. We adopt a GMM of 20 mixtures to serve as the model prior, and collect 4 trajectories every time for the update of the system dynamics and the linear Gaussian policy. We compare the proposed GPS model-based RL method with a series of popular model based and model free RL methods, in terms of their training and testing performance. We described the setting for the proposed method and briefly introduce the baseline algorithms and their settings in the following subsections.

\paragraph{Cross entropy method (CEM)} \cite{de2005tutorial} has been one of the most simple and popular policy search RL method for policy optimization. In order to optimize the parameterized policy $\pi_\theta$, the CEM adopts the assumption of Gaussian distribution of $\theta \sim \mathcal{N} (\mu, \sigma^2)$. It iteratively samples $\theta$ from the distribution, using which to collect sample trajectories, and then updates $\mu$ and $\sigma$ using the $\theta$'s that produces the best trajectories. In our implementation, since the CEM is also a policy search method, to make a fair comparison, we also collect 4 trajectories every time for policy update.

\paragraph{Model-free RL soft actor critic (SAC)} \cite{haarnoja2018soft} algorithm, which is currently the state of the art model free RL algorithm, with one of the best sample complexity and the convergence property among the model-free RL algorithms. The SAC maximizes both the expected reward (negative cost) and the entropy

\begin{align}
\max_\theta \sum_{t=0}^{T-1} E_{\pi_\theta} [-c(s_t, a_t) + \alpha H(\pi_\theta)]
\end{align}

The SAC adopts soft Bellman equation to solve for the optimal soft Q value function, resulting in a stochastic neural network policy. In our implementation, the policy network and the critic network are both fully connected neural networks with two hidden layers of 256 neurons. Each time step, we collect a batch size of 256 steps for the off policy model free RL training, and adopt a learning rate of 0.0003.

\subsection{Comparison and Discussion}

\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{part1_inside_policy/mbrl/figures/no_obs.png}
\caption{The training log of the guided policy search (GPS) and cross entropy methods (CEM) on the driving task without obstacles. The GPS based method converges faster and to a better driving policy compared to the CEM.}
\label{fig:GPS_CEM_no_obs}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{part1_inside_policy/mbrl/figures/w_obs.png}
\caption{The training log of the guided policy search (GPS) and cross entropy methods (CEM) on the driving task with obstacle. Similar to the task without obstacle, the GPS based method converges faster and to a better driving policy compared to the CEM.}
\label{fig:GPS_CEM_obs}
\end{figure}

As described in Section \ref{carla_setup}. The experiments are divided to two parts, driving without obstacles and with obstacles, since the two sets of tasks have different dimension of input and different cost functions. For both cases, the autonomous vehicle is randomly initiated from one of the three settings, the straight driving, $90\degree$ turning and roundabout entering. We run the proposed GPS based method and the baselines of CEM, SAC methods to learn the urban driving policies, and the figures below show the training log of the methods in comparison. For GPS and CEM, since the policies are linear Gaussian, we apply a PD controller as the initialization, with large variance. For the model free RL, the policies are neural networks, so we follow the pure random initialization. Therefore, the initial performances of the GPS and CEM are slightly better compared to the model free RL methods.

Fig. \ref{fig:GPS_CEM_no_obs} shows the training log of the policy search methods, the GPS and CEM methods on driving tasks without obstacles and Fig. \ref{fig:GPS_CEM_obs} shows the training log of the two methods in tasks with obstacles. It is shown that in both cases, the GPS method outperforms the CEM in terms of both the speed and the optimum of convergence. The GPS algorithms converges with only about 1000 steps of data, corresponding to 100 seconds driving, while the CEM takes roughly twice as much time to converge. In terms of the qualitative performance, the GPS policy (roughly -100k reward) can track the road lane more stably and can surpass the front vehicle when it affects the speed profile of the autonomous vehicle, while the CEM methods (roughtly -200k reward) can make uncomfortable steering actions, and also sometimes collide with the obstacle or drive out of the road.

Fig. \ref{fig:GPS_CEM_SAC} shows the comparison of the model based and policy search methods with the state of the art model-free RL method of SAC. It is shown that the model-free SAC method achieve a similar performance compared with our proposed GPS based method. However, the sample efficiency property of our proposed model based method is 100 times better, since the SAC takes more than 100k steps to converge and GPS only took 1k steps to converge. Fig. \ref{fig:qualitative} is an example showing the qualitative performance of the GPS policy in a case where the ego vehicle actively changes its lane to surpass the obstacle vehicle.

\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{part1_inside_policy/mbrl/figures/comparison.png}
\caption{The training log of the guided policy search (GPS) and cross entropy methods (CEM) in comparison with the soft actor critic (SAC) model free RL method on tasks without obstacles. The model free RL can learn satisfying driving policy, but it takes mode than 100k steps of data for training. That is, the model based method is 100x more sample efficient.}
\label{fig:GPS_CEM_SAC}
\end{figure}

\begin{figure}[!htb]
\minipage{0.12\textwidth}
  \includegraphics[width=\linewidth]{part1_inside_policy/mbrl/figures/1.png}
\endminipage\hfill
\minipage{0.12\textwidth}
  \includegraphics[width=\linewidth]{part1_inside_policy/mbrl/figures/2.png}
\endminipage\hfill
\minipage{0.12\textwidth}%
  \includegraphics[width=\linewidth]{part1_inside_policy/mbrl/figures/3.png}
\endminipage
\minipage{0.12\textwidth}%
  \includegraphics[width=\linewidth]{part1_inside_policy/mbrl/figures/4.png}
\endminipage
\caption{Qualitative performance of the GPS policy in a case where the ego vehicle actively changes its lane to surpass the obstacle vehicle. This task involves high level decision and planning intelligence, which is hard to learn.}
\label{fig:qualitative}
\end{figure}

To summarize, as a model-based RL approach, when applied in urban autonomous driving, the GPS has the advantages of higher sample efficiency, better interpretability, and greater stability. The experiments validate the effectiveness of the proposed method to learn robust driving policy for urban driving in Carla. We also compare the proposed method with other policy search and model-free RL baselines, showing 100x better sample efficiency of the GPS compared with the model-free RL baseline, as well as that GPS can learn policies for harder tasks that the baseline methods can hardly learn

==> part1_inside_policy/mbrl/sections/5Results_Discussion.tex <==
\section{Model-free RL: State Representation Formulation}
\label{sec:end}

In this section, we investigate the performance comparisons between the usage of different state encoding for the representation of the highly interactive urban driving scenario. As described in section \ref{carla_setup}, the Carla simulator could provide a full state feature vector of the ego vehicle and the surrounding vehicles, as well as simulated sensor output, such as the front camera and the lidar images. With an end-to-end model-free RL formulation, the encoding of the complicated and interactive driving scenario is very important for the understanding of the situation and for the control of the ego vehicle. We investigate a series of candidate representations and validate the graph neural network (GNN) based representation encoding is the best choice in terms of policy learning performance.

\subsection{Graph Neural Network Representation Formulation}

Graph neural network (GNN) has recently draw significant attention in the research community thanks to its capability of capturing the relational biases between entities in complicated systems \cite{kipf2018neural} \cite{battaglia2018relational}. In our autonomous driving task, we also introduce the usage of GNN to serve as the representation extractor to encode the interaction information between the traffic participants. The interactive driving scenario is first described using a graph formulation, with vertex states $V_i$ representing each of the traffic participants, and edge states $E_{i, j}$ represents the relationship between two traffic participants. Fig. \ref{fig:gnn_driving} shows the graph representation formulation for the driving case. For the sake of simplicity, in our formulation, the edges are directed edges, and only the effect of the surrounding vehicles towards the ego vehicle are considered. That is, there is no directed edges from the ego vehicle towards the surrounding vehicles, or between the surrounding vehicles. The vertex state stores the position and velocity of the corresponding vehicle, and the vertex stores the relational distance and velocity difference between the two vehicles.

\begin{figure}
\centering
\includegraphics[width=\linewidth]{part1_inside_policy/mbrl/figures/gnn_driving.png}
\caption{The graph representation of the driving scenario with multiple traffic participants.}
\label{fig:gnn_driving}
\end{figure}

In the graph neural network, the initial graph formulation is then processed using convolutional graph layers, in which a vertex update operation and an edge update operation are proceeded iteratively. In edge update, the current edge and its starting and ending vertices are fed into a fully connected network to produce the next edge feature. In vertex update, the current vertex and all incoming edges are fed into a fully connected network to produce the next vertex feature. The graph convolutional layer is elaborated in Algorithm \ref{algo:gcn}

\begin{algorithm}
\SetAlgoLined
Input: kth graph layer $V_i^k, i \in \{0, ..., n\}$, $E_{i, j}^k, (i, j) \in E$, fully connected networks: $\phi_\theta_e$, $\phi_\theta_v$\\
\For{$(i, j) \in E$}{
  $E_{i, j}^{k+1} = \phi_\theta_e(E_{i, j}^k, V_i^k, V_j^k)$
}
\For{$i \in \{0, ..., n\}$}{
  let $E_i^{k+1} = \Sigma_{(i, j) \in E} E_{i, j}^{k+1}$\\
  $V_i^{k+1} = \phi_\theta_v(V_i^{k}, E_i^{k+1})$
}
Return: (k+1)th graph layer $V_i^{k+1}, i \in \{0, ..., n\}$, $E_{i, j}^{k+1}, (i, j) \in E$
\caption{Graph Convolutional Layer}
\label{algo:gcn}
\end{algorithm}

\subsection{Comparison between Other Representation Formulations}

The proposed graph-based representation formulation is compared with the two following baselines:

\paragraph{Sensor data:} the Carla simulator provide rich simulated sensor data including the front view camera image and the lidar image as shown in Fig. \ref{fig:carla_obs}. We concatenate the camera image and the lidar image along the channel axis, and feed it into a convolutional neural network feature extractor.
\paragraph{State vector:} To illustrate the effectiveness of the graph structure, we compare it with a full state input of all the traffic participants, which is fed into a fully connected network for feature extraction. Since number of the surrounding vehicles can be varying, we define a state vector with enough entries for at most 10 vehicles, and feed the detectable vehicles to the state vector. If there is not enough vehicles within detectable distance, we append 0's to the remaining entries.

We train policy networks using the three state representations using soft actor critic for 35k steps till convergence. Fig. \ref{fig:gnn_performance} shows the comparison of the performance with different representations. The training logs show that the graph neural network based representation achieves superior performance compared with the sensor data and the state vector. Using the sensor data version representation, sac cannot learn a driving policy that successfully navigate in the Carla simulator, while the state vector version policy improves slower than the graph version policy. The final performance is also below that of the proposed graph version policy. We also validated the performance of the graph neural network with varying number of surrounding vehicles by training two separate policies within Carla scenarios with and without varying number of surrounding vehicles. Training logs in Fig. \ref{fig:gnn_diff_num_vh} show that the policy trained with fixed number of surrounding vehicles improves to convergence faster, while the policy trained with random number of surrounding vehicles also reaches similar performance in the end. Therefore, we validate that the graph neural network representation is helpful for encoding the information within a complicated driving scenarios multiple vehicles. Also, the graph formulation is capable of handling a varying number of entities.

\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{part1_inside_policy/mbrl/figures/gnn_performance.png}
\caption{Training log comparison of the graph representation and the baseline representations.}
\label{fig:gnn_performance}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{part1_inside_policy/mbrl/figures/gnn_diff_num_vh.png}
\caption{Training log comparison of the graph representation policy trained in scenarios with and without varying number of surrounding vehicles.}
\label{fig:gnn_diff_num_vh}
\end{figure}
